Universal end-compactifications of locally finite graphs

We construct a locally finite connected graph whose Freudenthal compactification is universal for the class of completely regular continua, a class also known in the literature under the name thin or graph-like continua.

==> tree.tex <==
\begin{tikzpicture}[scale=0.5]

    
    \foreach \point in {
         (4.0, 0),
 (8.0, 2),
 (10.0, 4),
 (11.0, 6),
 (9.0, 6),
 (6.0, 4),
 (7.0, 6),
 (5.0, 6),
 (0.0, 2),
 (2.0, 4),
 (3.0, 6),
 (1.0, 6),
 (-2.0, 4),
 (-1.0, 6),
 (-3.0, 6)
    } {
        \def\this{vertex-\point}
        \node (\this) at \point  [circle,fill=black, inner sep=1.5pt] {} ;
    }
    
% Invisible ellipse to fix height offset with blowup picture
\draw [opacity=0](-3.0, 6) ellipse (0.8999999999999999cm and 0.3cm);
    
% Edges
\draw[thick] (4.0, 0)--(8.0, 2);
\draw[thick] (8.0, 2)--(10.0, 4);
\draw[thick] (10.0, 4)--(11.0, 6);
\draw[thick] (10.0, 4)--(9.0, 6);
\draw[thick] (8.0, 2)--(6.0, 4);
\draw[thick] (6.0, 4)--(7.0, 6);
\draw[thick] (6.0, 4)--(5.0, 6);
\draw[thick] (4.0, 0)--(0.0, 2);
\draw[thick] (0.0, 2)--(2.0, 4);
\draw[thick] (2.0, 4)--(3.0, 6);
\draw[thick] (2.0, 4)--(1.0, 6);
\draw[thick] (0.0, 2)--(-2.0, 4);
\draw[thick] (-2.0, 4)--(-1.0, 6);
\draw[thick] (-2.0, 4)--(-3.0, 6);

\end{tikzpicture}

